The complexity of verifying the release-acquire semantics over register machines

The Release-Acquire (RA) semantics and its variants are some of the most fundamental models of concurrent semantics for architectures, programming languages, and distributed systems. Several steps have been taken in the direction of testing such semantics, where one is interested in whether a single program execution is consistent with a memory model. The more general verification problem, i.e., checking whether any allowed program run is consistent with a memory model, has still not been studied as much. The purpose of this work is to bridge this gap. We tackle the verification problem, where, given an implementation described as a register machine, we check if any of its runs violates the RA semantics or its Strong (SRA) and Weak (WRA) variants. We show that verifying WRA in this setup is in O(n5 ), while verifying the RA and SRA is PSPACE complete. This both answers some fundamental questions about the complexity of these problems, but also provides insights on the expressive power of register machines as a model.

==> RelatedWork.tex <==

%
In their seminal work \cite{DBLP:journals/siamcomp/GibbonsK97}, Korach and Gibbons showed consistency testing under the SC semantics is NP-hard.
%
Alur et al. showed that the verification problem under the SC semantics \cite{DBLP:journals/iandc/AlurMP00} is undecidable, albeit for a data-dependent implementation model. Hence, one that registers machines cannot capture.

%


Several examples of protocols (\cite{DBLP:journals/dc/AhamadNBKH95,DBLP:conf/ppopp/PerrinMJ16}) are designed to enforce different consistency models.
Such works guarantee the designed mechanisms' correctness and provide a good baseline for implementing practices.
However, they do not produce uniform frameworks or algorithms to answer the general consistency-checking question. 




Bouajjani et al. \cite{DBLP:conf/popl/BouajjaniEGH17} consider the verification problem for semantics, which is equivalent to \wrasem, but with a model that allows unbounded numbers of pending messages.
%
They show the problem is \EXPSPACE-complete.



Another primary direction is verifying \emph{single runs}, expressed as sequences of memory access events, to determine whether that run satisfies a consistency model. 
%This version of verification is related to \textit{testing}.
%In this setting, it is essential to correctly detect that a specific sequence of accesses is violating the semantics of the memory model. 
This problem is quite complex in general, as, for at least all the memory models studied in this work, there is an unbounded number of possible reorderings of the observed events from one local view to the other. 
Several works consider the testing problem under the \rasem semantics \cite{DBLP:journals/pacmpl/AbdullaAJN18,DBLP:journals/pacmpl/TuncA0K0P23}.
%
%In these works, we also encounter the assumption of \emph{data independence} \cite{POPL_Wolper86_data_independence} (which is a very realistic assumption stating that the content of the memory accesses does not affect the execution \cite{DBLP:conf/popl/BouajjaniEGH17}). 
% The problem becomes easier to tackle. 
%Specifically, in this case, one can study only the case of differentiated runs, i.e. runs where all the data is distinct, and yet produce results for any run. 
%This is because we can replace all data values with symbolic ones, without affecting the execution at all. 
%
These works show that the testing problem has polynomial complexity for \rasem.
%
Bouajjani et al. \cite{DBLP:conf/popl/BouajjaniEGH17} show that the testing problem for the \wrasem semantics has polynomial complexity. 


Both works focus on providing a specific implementation or verifying a single run from an unknown implementation. 
Our results show that the verification problem wrt.\ register machines also has polynomial complexity (albeit with a higher degree).
%c






==> doc/makefile <==
# $Id: makefile 282 2026-01-08 05:54:22Z rishi $

file=elsdoc


all: pdf out 
	make pdf
	make pdf

#out:
#	if  [ -f $(file).out ] ; then cp $(file).out tmp.out; fi ;
#	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ;

out:
	if  [ -f "$(file).out" ] ; then cp "$(file).out" tmp.out; fi ; 
	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ; 
	sed -i 's/{\\376\\377/{/g' tmp.out ; 
	sed -i '/dtxmark/s/\\000//g' tmp.out
	sed -i 's/\\040/ /g' tmp.out ; 
	sed -i 's/\t/ /g' tmp.out

pdf:
	pdflatex $(file).tex

index:
	makeindex -s gind.ist -o $(file).ind $(file).idx 

changes:
	makeindex -s gglo.ist -o $(file).gls $(file).glo

xview:
#	xpdf -z 200 $(file).pdf &>/dev/null
	open -a 'Skim.app' $(file).pdf 

view:
	open -a 'Adobe Reader.app' $(file).pdf

ins:
	latex $(file).ins 

diff:
	diff $(file).sty ../$(file).sty |less

copy:
	cp $(file).sty ../



==> egraphs.tex <==
In this section, we formulate the notion of execution graphs (egraphs) and then define an operation that allows building egraphs incrementally by adding new events.
%
By interpreting the runs of a register machines as execution graphs, we define the set of execution graphs that the register machine generates.
%
In the \cref{sec:memory_models}, we use the set of generated execution graphs to judge whether the machine satisfies a given consistency model.

\subsection{Definition}
The nodes of an egraph are events.
%
An {\it event} $\event$ is of the form $\eventof\ttype\thread\eid\xvar$ where $\ttype\in\set{\wtype,\rtype}$ is the type of the event (write or read), $\thread\in\threadset$ is the thread performing the event, $\eid\in\nat$ is the event identifier (unique per thread), and $\xvar\in\varset$ is the variable on which $\thread$ conducts the event.
%
We define $\typeattrof\event:=\ttype$, $\threadattrof\event:=\thread$, $\idattrof\event:=\eid$, and $\varattrof\event:=\xvar$.
%
%
We will use a set $\initeventset=\setcomp{\xinitevent\xvar}{\xvar\in\varset}$ of {\it initial} write events, where $\xinitevent\xvar$ represents a dummy event writing the initial value $\zero$ to $\xvar$.
We assume that the initial events do not belong to any threads.
%
We use $\eventset$ to denote the set of all events.
%
%

%
For a set of events $\events\subseteq\eventset$, we define the relation 
$\mkrelof\events:=\setcomp{\tuple{\event,\event}}{\event\in\events}$, i.e., it is the restriction of the identity relation to the set of events in $\events$.
%
For $\ttype\in\set{\wtype,\rtype}$, we define the relation $\mkrelof\ttype:=\setcomp{\tuple{\event,\event}}{\typeattrof\event=\ttype}$, i.e. it is the restriction of the identity relation to the set of events of type $\ttype$.
%
Similarly, for a thread $\thread\in\threadset$, we define the relation $\mkrelof\thread:=\setcomp{\tuple{\event,\event}}{\threadattrof\event=\thread}$.
%
Sometimes, we view these relations as sets and write, e.g.,  $\event\in\mkrelof\rtype$ to denote that $\event$ is of type $\rtype$.
%
We also consider Boolean combinations of these relations, so we write $\mkrelof{\events\land\rtype}$ to denote the set of events in $\events$ of type $\rtype$.
%
Fix a set $\events: \initeventset\subseteq\events\subseteq\eventset$ of events.
%
\begin{itemize}
    \item A {\it program-order} on $\events$ is a relation $\porel$ defined as a union $\cup_{\thread\in\threadset}\,\xporel\thread$ such that  $\xporel\thread$ is a total order on the set of events in $\mkrelof{\events\land\thread}$.
    %
    In other words, $\porel$ totally orders all the events in $\events$ belonging to each thread.
    \item  A {\it reads-from} relation $\rfrel\subseteq\mkrelof{\events\land\wtype}\times\mkrelof{\events\land\rtype}$ assigns to each read event $\revent$ a write event $\wevent$ in $\events$ such that $\varattrof\revent=\varattrof\wevent$.
    %
    We will write, $\wevent\mkrelof\rfrel\revent$ to mean that $\revent$ takes its value from $\wevent$. 
    \item   
    A {\it coherence-order} on $\events$ is a relation $\corel$ defined as a $\cup_{\xvar\in\varset}\,\xcorel\xvar$ such that $\xcorel\xvar$ is a partial order on the set of write events on $\xvar$.
    %
    We require that $\xinitevent\xvar$ is the smallest element in the sub-relation  $\xcorel\xvar$.
    %
    A {\it total-coherence-order},  $\corel$ on $\eventset$ is a coherence-order in which the $\xvar$-sub-relations are total. 
    % 
    In other words, $\corel=\cup_{\xvar\in\varset}\,\xcorel\xvar$ and $\xcorel\xvar$ is a total order on the set of write events on $\xvar$.
    %
    
\end{itemize}
%
%We use $\rfrelsof\events$  and $\corelsof\events$ to denote the sets of read-from resp.\ coherence-order relations on $\events$.
%\patodo{The last sentence to be removed?}
%
We also define the {\it happens-before} relation $\hbrel:=(\porel\cup\rfrel)^+$. 
%and
%the {\it causally-before} relation $\xcbrel\xvar:=\rclosureof{(\xcorel\xvar)}\compose\hbrel$, $\cbrel:=\cup_{\xvar\in\varset}\xcbrel\xvar$.
An {\it execution graph} $\egraph$ is a tuple $\tuple{\events,\porel,\rfrel,\corel}$ where:
(i)
$\events\subseteq\eventset$ is a set of events such that $\initeventset\subseteq\events$,
(ii)
$\porel$ a program-order on the set $\events$,
(iii)
$\rfrel$ is a  reads-from relation on $\events$, and
(iv)
$\corel$ is a coherence-order relation on $\events$.
%
A {\it total egraph}, is an  egraph in which  the coherence-order relation is total on each variable $\xvar$.
%
For a relation $\rel$, an event $\event\in\events$, and a thread $\thread\in\threadset$, we write $\event\mkrelof\rel\thread$  if $\event\mkrelof\rel\pevent$ for some $\pevent\in\mkrelof{\events\land\thread}$.
The initial egraph is defined by $\initegraph:=\tuple{\initeventset,\emptyset,\emptyset,\emptyset}$, i.e., it only contains the initial events, and all its relations are empty.

\subsection{Adding Events}
We define an operation $\addevent$ that adds a new event to an egraph, according to the rules given in \cref{add:event:fig}.
\begin{figure}
    \centering
    \includegraphics[scale=0.72]{{Figures/Egraphs/rules}}
\caption{The rules for adding events to an egraph. A write event only causes an update to the program order relation $\porel$, while a read event creates also $\rfrel$ and $\corel$ edges. Since $\corel$ edge are added only when necessary, then the resulting $\corel$ is a partial one.}
\label{add:event:fig}
\end{figure}
If the new event $\wevent$ is a write event performed by a thread $\thread$, we add $\wevent$ to the set of events.
%
We require the identifier $\eid$ of $\event$ to reflect its order among the events of $\thread$ wrt.\ the $\porel$-relation.
%
More precisely, we require $\eid$ to be one plus the number of $\thread$-events.
%
Adding a write event does not affect the $\rfrel$- and $\porel$-relations.
%

If the new event to be added is a read even $\revent$, then we also need to provide a write event $\wevent$ that already belongs to $\events$ from which $\revent$ will read its value.
%
The events $\revent$ and $\wevent$ should have identical variables.
%
We modify the $\porel$-relation in the same manner as we did for write events.
%
We modify the $\rfrel$-relation by adding the new pair $\tuple{\wevent,\revent}$ indicating that $\revent$ is reading from $\wevent$.
%
Finally, we update the coherence-order so that we maintain the invariant that the latter is a modification-order.
%
To that end, we consider $\wevent$ and $\revent$ to be sources and targets, and then search for write events $\pwevent$ that can serve as victims, i.e., $\pwevent\mkrelof\hbrel\revent$% (see \cref{sec:overview})
.
%
We add each such a pair $\tuple{\pwevent,\wevent}$ to the $\corel$-relation.

%


\subsection{From Runs to Egraphs}
\label{Run:Egraph:subsection}
%
\begin{wrapfigure}[13]{R}{0.5\textwidth}
  \begin{center}
    \includegraphics[scale=0.72]{Figures/mkEgraphs/rules}
  \end{center}
%\begin{gather*}
%  \scalebox{0.75}{
%\oneinfer
%    {
%    }
%    {
%      \tuple{\mystate,\regvalmapping}
%      \rmovesto\rmachine{\weventof\thread\xvar\areg\textcolor{red}{\sslash\val}}{}
%      \tuple{\pstate,\pregvalmapping}
%    }
%}
%\end{gather*}
\caption{The inference rules for deriving egraphs from runs.}
\label{run:egraph:fig}
\end{wrapfigure}
We associate each run $\run$ of a register machine with a corresponding egraph $\egraph:=\mkegraphof\run$.
%
We define the function $\mkegraph$ according to the rules of \cref{run:egraph:fig}.
%
If $\run$ is empty then $\egraph$ is equal to the initial egraph $\initegraph$.
%
Otherwise, we define $\egraph$ inductively by considering a run 
$\run\app\tuple{\istate1,\op,\istate2}$ whose last operation is $\op$.
%
More precisely, we add a new event to $\egraph$ according to $\op$.
%
If $\op=\wopof\thread\xvar\areg$ is a write operation, we add a new write event $\wevent$ to $\egraph$.
%
The event $\wevent=\weventof\thread\eid\xvar$ has the same thread and variable attributes as $\op$.
%
However, we do not include the register $\areg$ in the definition of $\event$.
%
Furthermore, we add the event identity $\eid$.
%
To ensure $\eid$ is unique among the events of $\thread$ in $\events$, we define $\eid$ to be the number of $\thread$-events in $\events$ plus one.
%
Once we have created $\wevent$ we add it to $\egraph$ using the $\addevent$ operation (\cref{add:event:fig}).
%
We handle the case of read events similarly.
%
However, here, we have also to provide the write $\wevent$ from which the new event $\revent$ reads its value.
%
To that end, we define the function
$\jj:=\max\setcomp{\ii}{\wposition\run\ii\in\mkrelof{\wtype\land\areg}}\cup\set0$.
%
If $\jj=0$ then we define $\lastwof\run\areg:=\initeventof\xvar$.
%
If $\jj>0$, we know that $\wposition\run\jj$ is of the form $\wopof\thread\xvar\areg$.
%
We define $\lastwof\run\areg:=\weventof\thread\xvar\kk$ where $\kk:=\sizeof{\run\land\thread}$.
%
Intuitively, the operation returns the latest operation that writes to the register $\areg$.
%
However, it is possible that this last operation was writing to a variable other than $\xvar$, something that is not a valid behavior, and it is now allowed by the semantics of execution graphs (\cref{add:event:fig}). 
We verify that this is not the case for a given register machine $\rmachine$ in \cref{sec:mismatched_vars}. 


==> experiments.tex <==
We have implemented the algorithms of \cref{sec:algorithms} in a prototype tool that inputs a register machine, and checks whether it satisfies the semantics of $\wrasem$, $\rasem$, and $\srasem$.
The verification is done in sequence, as if one of the models is not respected, then neither are the subsequent, stronger, models.
When our tool detects a violation it prints the series of transitions that constitute the run which would create an illegal execution graph. 

The implementation has been tested on several small examples from \cite{DBLP:conf/popl/LahavGV16} and \cite{DBLP:conf/cav/AbdullaAGKV23}, %that each represent executions that violate some form of consistency,
the well known MOSI and MSI cache protocols, and two larger examples
of
register machines
that express the policies for distributed memory accesses.
The last two correspond to the implementations of causally consistent distributed processes from
\cite{DBLP:journals/dc/AhamadNBKH95}, and \cite{DBLP:conf/ppopp/PerrinMJ16}. For those, the expected, and acquired, result was for the register machine protocol to satisfy $\wrasem$ but not $\rasem$, as causal consistency in this setting coincides with $\wrasem$ \cite{DBLP:conf/popl/BouajjaniEGH17}.
%The last use case is a register machine we defined to allow for $\rasem$ consistent memory accesses between a set of communicating processes.
The last two use cases also contribute a methodology for modeling existing protocols as register machines, so that the verification can be performed.
The state space of the produced register machine is of course very large, as often it needs to encode in the states not only information about the variables of a distributed protocol, but information about the content of
those variables.
However, our implementation did manage to handle all of the included examples for at least two threads and two variables, which is enough to provide useful insights for the general case, and acts as a first step towards acquiring an implementation with larger capacity.
The implementation is openly available, hosted on Github \cite{codelink}.


We continue with a presentation of our experiments and the performance of the algorithm.
To begin we first tested our algorithm on known litmus test style examples of execution graphs that separate or characterize various memory models.
To do so, we created several register machines that could produce executions whose execution graphs matched those patterns.
Examples of these are \cref{not:WRA:aut:fig}, \ref{ra:not:sra:fig}, and \ref{fig:exra}.
\begin{comment}
When searching for hidden read violations in the register machine presented in \cref{fig:exra}, the rules are matched as follows.
\begin{enumerate}
    \item Each output edge is matched in $\bluecircled{1}$, adding
    $\alpha(x, a_2) \oplus \tuple{q_3, \theta_1}$ and
    $\alpha(x, a_1) \oplus \tuple{q_2, \theta_2}$.
    \item
    The output edge $\outopof{\theta_2}{x}{a_1}$ together with the tuple $\tuple{q_3, \theta_1} \in \alpha(x, a_2)$ matches rule $\bluecircled{17}$, adding $\alpha(x, a_2) \oplus \tuple{q_2, \theta_1}$.
    \item
    The input edge $\inopof{\theta_2}{x}{a_2}{-}$ together with $\tuple{q_2, \theta_2} \in \alpha(x, a_1)$ matches rule $\bluecircled{4}$, adding
    $\beta(x, a_1) \oplus \tuple{q_1, \theta_2}$
    \setcounter{evalctr}{\value{enumi}}
\end{enumerate}
Which concludes the saturation for$\wrasem$. We proceed by adding the rules for$\rasem$, and perform saturation,
\begin{enumerate}
\setcounter{enumi}{\value{evalctr}}
\item
    The input edge $\inopof{\theta_2}{x}{a_2}{-}$ together with
    $\tuple{q_2, \theta_1} \in \alpha(x, a_2)$ and
    $\tuple{q_2, \theta_2} \in \alpha{x, a_1}$ matches rule $\bluecircled{21}$, adding
    $\beta(x, a_1) \oplus \tuple{q_1, \theta_1}$
\item
    The input edge $\inopof{\theta_1}{x}{a_1}{-}$ together with $\tuple{q_1, \theta_1} \in \beta(x, a_1)$ matches rule $\bluecircled{10}$,
    adding $\failconf$.
\end{enumerate}
 At which point we conclude the register machine guarantees$\wrasem$ but not$\rasem$.
\end{comment}
%\begin{figure}
%\scalebox{0.65}{
%    \begin{tikzpicture}
%
%        \node[state, initial] (q0) at (0,0) {$q_0$};
%        \node[state] (q1) at (3,0) {$q_1$};
%        \node[state] (q2) at (6, 0) {$q_2$};
%        \node[state] (q3) at (9, 0) {$q_3$};
%        \node[state] (q4) at (12, 0) {$q_4$};
%        \node[state] (q5) at (15, 0) {$q_5$};
%        \node[state] (q6) at (18, 0) {$q_6$};
%
%        \draw[-stealth] (q0) to[bend left] node[above,midway] {$\inopof{\theta_1}{x}{a_1}{-}$} (q1);
%        \draw[-stealth] (q1) to[bend left] node[above,midway] {$\inopof{\theta_2}{y}{b_1}{-}$} (q2);
%        \draw[-stealth] (q2) to[bend left] node[above,midway] {$\inopof{\theta_1}{y}{b_2}{-}$} (q3);
%        % Messed up order to not fill too much white
%        \draw[-stealth] (q4) to[bend left] node[above,midway] {$\outopof{\theta_1}{y}{b_1}$} (q5);
%
%        \draw[-stealth] (q3) to[bend left] node[above,midway]{$\inopof{\theta_2}{x}{a_2}{-}$} (q4);
%
%
%        \draw[-stealth] (q5) to[bend left] node[above,midway] {$\outopof{\theta_2}{x}{a_1}$}  (q6);
%    \end{tikzpicture}
%}
%    \caption{%
%    A register machine that produces the execution graph of \cref{fig:SRA_violation}. It satisfies $\wrasem$ and $\rasem$, but not $\srasem$, as there is a cycle in $\tclosureof{\mkrelof{\porel\cup\rfrel\cup\partcorel}}$.}
%    \label{fig:exsra}
%\end{figure}
We summarize all our tests in \cref{tab:tests}.
\begin{table}
\caption{Experimental data. Each test is parameterized by the number of processes, in parentheses. The tests were executed on an Intel Xeon Platinum 8168 processor with 48 physical cores, each clocked at 2.7GHz. The column ``Variations'' refers to the number of different register machines we implemented for producing the relevant execution graph.
The column ``Transitions'' refers to the number of transitions in each register machine.
Clearly, the number of transitions has an effect on the runtime, although we see that some of the protocols on the ``safer'' side terminate faster, as less tuples are created to keep track of ``dangerous'' paths. The MM results indicates that the protocol did not satisfy WRA, but does not have any mismatched variables. The parenthesis after a register machine signifies its parameters. For broadcast it is the number of threads, for MOSI and MSI it is (threads, variables), and for Vector Clock it is (threads, variables, queue length)}
\begin{tabular}{l|lllc}
    \hline
    Register machine & Variations & Runtime & Transitions & Weakest Violated Model \\
    \hline
    Out of order reads \cite{DBLP:conf/cav/AbdullaAGKV23} & 4 & 14ms & 6 & RA \\
    2+2W \cite{DBLP:journals/toplas/LahavB22} & 2 & 11ms & 7 & SRA \\
    MP \cite{DBLP:journals/toplas/LahavB22} & 1 & 1.9ms & 6 & WRA \\
    MP Trans \cite{DBLP:journals/toplas/LahavB22} & 1 & 2.2ms & 7 & WRA\\
    SB \cite{DBLP:journals/toplas/LahavB22} & 1 & 9.3ms & 7 & - \\
    SF \cite{DBLP:journals/toplas/LahavB22} & 1 & 4.6ms & 5 & RA \\
    WW \cite{DBLP:journals/toplas/LahavB22} & 1 & 5.29ms & 5 & RA \\
    WW MP \cite{DBLP:journals/toplas/LahavB22} & 1 & 12.3ms & 7 & - \\
    Oscillating \cite{DBLP:journals/toplas/LahavB22} & 3 & 6.44ms & 6 & SRA\\
    Broadcast (2) \ref{sec:bcast} & 1 & 4.5ms & 22 & RA \\
    Broadcast (3) \ref{sec:bcast} & 1 & 2.3s & 1889 & RA \\
  Vector Clock (2,1,2) \ref{sec:vclock} & 1 & 8.08s & 3564 & RA \\
  Vector Clock (2,2,2) \ref{sec:vclock} & 1 & 17m & 38496 & WRA\\
%    $\rasem$ protocol (2) \ref{sec:rasemex} & 1 & 24m & 1071 & SRA \\
    MOSI (4,2) & 1 & 48.7s & 2176 & - \\
    MSI (2, 1) & 1 & 86ms & 39 & - \\
    \hline
\end{tabular}
\label{tab:tests}
\end{table}

\subsection{Buffers, Fences and Applicability}
In order to model a buffer, we need to encode its contents as part of each state in the register machine; in other words, we may say that each state contains buffer contents, in addition to register contents. In our experiments, we have encoded this extra information as part of the state identifier. Using this encoding we can model fences as a sequence of transitions between intermediate states. Specifically, if a state $q_{i,j,k}$ has three \emph{messages} $i,j,k$ in its buffer, we will add a transition from $q_{i,j,k}$ to some other state $q'_{j,k}$ corresponding to handling this message. The edge on the transition is usually a copy edge, since a message in these buffers usually encode that there is a write that is yet to be seen by the receiving thread. Augmenting the states of register machine models with additional information allows for encode complex systems. In particular, cache protocols modeled with SLICC \cite{SLICC:94} can be encoded as register machine models in this way.

 \subsection{Distributed Memory}
 \label{sec:bcast}
The algorithm was used to test the protocol for a distributed memory system that satisfies causal consistency from \cite{DBLP:conf/ppopp/PerrinMJ16}. The protocol uses message parsing to send information to other processes.
Whenever a write by process $p$ occurs, $p$ will send a message to each other process containing the value of the write. The system operates with the assumption that if a process $p$ has received message $m$ before writing, each other process will receive the message $m$ before they receive the write message from $p$. For simplicity, we have defined some additional constraints on the system. Namely, the messages arrive instantaneously, they are sent in the same order every time, and a process may not perform any other input operations until its broadcast is complete.

A write operation on variable $x$ by process $p$ in the system consists of a series of steps. In the first, we atomically write the value into a special broadcast register $bc_p$ for process $p$, and copy it to the register $x_p$ -- the register representing the contents of variable $x$ on process $p$. Then, for each other process $p'$, we copy $x_{p'} := bc_p$, which corresponds to $p$ informing $p'$ of the write. Such a copy transition is only enabled if the receiving process has currently received all messages the writer had received when it started the write. This information -- from whom we last received a write -- is kept as part of a state in the register machine model. A register machine modeling this protocol for three processes is verified to satisfy $\wrasem$, but not $\rasem$.

\subsection{Vector Clocks}
\label{sec:vclock}
A second protocol for a causally consistent memory system is described in \cite{DBLP:journals/dc/AhamadNBKH95}.
It uses vector clocks to keep processes in sync. Whenever a process $p$ performs a write, it appends a message containing the value and $p$s current clocks to an outgoing queue. Nondeterministically, this message may get sent to other processes, in which case it is appended to the input queue of that process. The input queue may also be nondeterministically emptied by accepting a message and writing its contents locally. This transition, however, is only available if the message clocks and the clocks of the receiving process are sufficiently in sync. This last condition is what makes the broadcast \emph{causal}, as described in \cite{DBLP:journals/dc/AhamadNBKH95}.

However, as the behavior of the protocol depends on the actual values in memory -- the vector clocks -- these values need to be kept as part of the states. Since the vector clocks are unbounded, they have to be limited to analyze. In order to preserve the possibility of infinite executions with bounded vector clock values, the states are connected through a disjoint copy operation -- effectively a skip operation -- that decrements all vector clocks by 1. Through this transition the important part of the clocks is kept; their relation to one another.


==> fig1.tex <==
\begin{figure}
  \begin{subfigure}[h]{0.4\linewidth}
    \scalebox{0.8}{
      \begin{tikzpicture}[initial text=,]
        \node[state, initial] (q0) at (0, 0) {$q_0$};
        \node[state] (q1) at (3, 0) {$q_1$};

        \node[fill=lightgray] (lb) at (-2, 0) {$\mathcal{M}_1$};
        
        \draw[-stealth] (q0) to[bend left] node[above,midway] {$\wopof{\theta}{x}{a}$} (q1);
        \draw[-stealth] (q1) to[bend left] node[below,midway] {$\wopof{\phi}{x}{b}$} (q0);

        \draw[-stealth] (q0) to[loop above] node[above,midway] {$\ropof{\theta}{x}{b}$} (q0);
        \draw[-stealth] (q0) to[loop below] node[below,midway] {$\ropof{\phi}{x}{a}$} (q0);

        \draw[-stealth] (q1) to[loop above] node[above,midway] {$\wopof{\theta}{x}{a}$} (q1);
      \end{tikzpicture}
      }
  \end{subfigure}
  \begin{subfigure}[h]{0.4\linewidth}
    \scalebox{0.8}{
    \begin{tikzpicture}
      \node (s1) at (0,2) {$\tuple{q_0, 0, 0}$};
      \node (s2) at (4,2) {$\tuple{q_1, 1, 0}$};
      \node (s3) at (8,2) {$\tuple{q_1, 2, 0}$};
      \node (s4) at (8,0) {$\tuple{q_0, 2, 3}$};
      \node (s5) at (4,0) {$\tuple{q_0, 2, 3}$};
      \node (s6) at (0,0) {$\tuple{q_0, 2, 3}$};

      \node[fill=lightgray] (lb) at (4, 1) {$\rho$};

      \draw[-stealth] (s1) to node[above, midway] {$\wopof{\theta}{x}{a}\textcolor{red}{\sslash1}$} (s2);
      \draw[-stealth] (s2) to node[above, midway] {$\wopof{\theta}{x}{a}\textcolor{red}{\sslash2}$} (s3);
      \draw[-stealth] (s3) to node[left, midway]  {$\wopof{\phi}{x}{b}\textcolor{red}{\sslash3}$} (s4);
      \draw[-stealth] (s4) to node[below, midway] {$\ropof{\phi}{x}{a}\textcolor{red}{\sslash2}$} (s5);
      \draw[-stealth] (s5) to node[below, midway] {$\ropof{\theta}{x}{b}\textcolor{red}{\sslash3}$} (s6);
    \end{tikzpicture}
    }
  \end{subfigure}
  \caption{A register machine $\irmachine1$ and a run $\run$ of $\irmachine1$}
  \label{fig:rmachine_and_run}
\end{figure}


==> fig2.tex <==
\begin{figure}[]
  \begin{subfigure}[h]{0.6\linewidth}
    \scalebox{0.7}{
    \begin{tikzpicture}[every edge/.style={-stealth}]
      \node[state] (q0) at (0,6) {$q_0$};
      \node[state] (q1) at (-2,4) {$q_1$};
      \node[state] (q2) at (2,4) {$q_2$};
      \node[state] (q3) at (-4,2) {$q_3$};
      \node[state] (q4) at (0,2) {$q_4$};
      \node[state] (q5) at (4,2) {$q_5$};
      \node[state] (q6) at (-2,0) {$q_6$};
      \node[state] (q7) at (2,0) {$q_7$};

      %Loops
      \draw[-stealth] (q0) to[loop above] (q0);
      \draw[-stealth] (q1) to[loop right] (q1);
      \draw[-stealth] (q2) to[loop left] (q2);
      \draw[-stealth] (q3) to[loop left] (q3);
      \draw[-stealth] (q4) to[loop above] (q4);
      \draw[-stealth] (q5) to[loop right] (q5);
      \draw[-stealth] (q6) to[loop below] (q6);
      \draw[-stealth] (q7) to[loop below] (q7);

      % straight edges
      \draw[-stealth] (q0) to (q1);
      \draw[-stealth] (q0) to (q2);

      \draw[-stealth] (q1) to (q3);
      \draw[-stealth] (q1) to (q4);

      \draw[-stealth] (q2) to (q4);
      \draw[-stealth] (q2) to (q5);

      \draw[-stealth] (q3) to (q6);
      
      \draw[-stealth] (q4) to (q6);
      \draw[-stealth] (q4) to (q7);

      \draw[-stealth] (q5) to (q7);

      \draw[-stealth] (q6) to (q5);
      \draw[-stealth] (q7) to (q3);

      % Curvy edges
      \draw[-stealth] (q3) to[bend left=45] (q0);
      \draw[-stealth] (q5) to[bend right=45] (q0);

      \draw[-stealth] (q7) to[bend right=45] (q5);
      \draw[-stealth] (q6) to[bend left=45] (q3);
    \end{tikzpicture}
    }
  \end{subfigure}
  \begin{subfigure}[h]{0.4\linewidth}
    \scalebox{0.7}{\begin{tabular}{ll}
      $\ell_{00}:~\wopof{\theta}{x}{a}$ &$\ell_{33}:~\ropof{\theta}{x}{a}$\\
      $\ell_{00}:~\wopof{\phi}{x}{b}$ &$\ell_{33}:~\ropof{\phi}{x}{a}$\\
      $\ell_{01}:~\ropof{\theta}{x}{b}$ &$\ell_{30}:~\wopof{\theta}{x}{a}$\\
      $\ell_{02}:~\ropof{\phi}{x}{a}$ &$\ell_{36}:~\wopof{\phi}{x}{b}$\\
      \\
      $\ell_{11}:~\ropof{\theta}{x}{b}$ &$\ell_{55}:~\ropof{\theta}{x}{b}$\\
      $\ell_{11}:~\wopof{\phi}{x}{b}$ &$\ell_{55}:~\ropof{\phi}{x}{b}$\\
      $\ell_{13}:~\wopof{\theta}{x}{a}$ &$\ell_{50}:~\wopof{\theta}{x}{a}$\\
      $\ell_{14}:~\ropof{\phi}{x}{a}$ &$\ell_{57}:~\wopof{\phi}{x}{b}$\\
      \\
      $\ell_{22}:~\ropof{\phi}{x}{a}$ &$\ell_{66}:~\ropof{\theta}{x}{a}$\\
      $\ell_{22}:~\wopof{\theta}{x}{a}$ &$\ell_{66}:~\ropof{\phi}{x}{a}$\\
      $\ell_{23}:~\wopof{\phi}{x}{b}$ &$\ell_{63}:~\wopof{\theta}{x}{a}$\\
      $\ell_{24}:~\ropof{\theta}{x}{b}$ &$\ell_{65}:~\wopof{\phi}{x}{b}$\\
      \\
      $\ell_{44}:~\ropof{\theta}{x}{b}$ &$\ell_{77}:~\ropof{\theta}{x}{b}$\\
      $\ell_{44}:~\ropof{\phi}{x}{a}$ &$\ell_{33}:~\ropof{\phi}{x}{b}$\\
      $\ell_{46}:~\wopof{\theta}{x}{a}$ &$\ell_{75}:~\wopof{\theta}{x}{a}$\\
      $\ell_{47}:~\ropof{\phi}{x}{b}$ &$\ell_{73}:~\wopof{\phi}{x}{b}$\\ 
    \end{tabular}
    }
  \end{subfigure}
\caption{The reactive version of the $\irmachine1$ of \cref{fig:rmachine_and_run}. The labels $\ell_{i,j}$ describe transitions from state $\qstate_i$ to $\qstate_j$. As we will see later, both this version and the original $M_1$, satisfy $\wrasem$.} \label{WRA:aut:fig}
\end{figure}


==> memory_models.tex <==


A declarative memory model is formulated as a collection of constraints on execution graphs, which
determine the consistent execution graphs—the ones allowed by the model. Each execution graph
describes a (partially ordered) history of a particular program run. 

In this section, we formulate the variants of causal consistency discussed in this paper as declarative models: Weak Release/Acquire (WRA), Release/Acquire (RA), and Strong Release/Acquire
(SRA).
All mentioned memory models are weaker than SC, and allow for less restrictive memory accesses. SC requires that as soon as some value has been written in some variable, this is immediately visible to all threads. 
The models we study instead allow for several threads to still view older values written in the variable, until they become ``aware'' of a new write on some path that ``hides'' the old value.

%Starting from the strongest model, that is, $\srasem$, we have that on an execution graph $\egraph$, a read event $\revent$ of a thread is aware of a write $\wevent$ on variable $\xvar$, if  there is any path on $\egraph$ that connects $\wevent$ to $\revent$. 
%$\wevent$ becomes hidden when there exists another write event $\wevent'$ on $\xvar$ on the path connecting  $\wevent$ to $\revent$. 
%Note here that the path might involve $\xcorel\yvar$ edges. Clearly, a write event might have been read by a thread, while another thread might still be reading a previous one. 
%
%RA respectively weakens this requirement to paths where the $\corel$ edges involved are for the same variable. 
%Again note that a read-from edge is not labelled with a variable, and thus $\rasem$-paths can use $\rfrel$ edges which connect reads a writes on variables other than $\xvar$. 
%Finally, $\wrasem$ weakens this requirement even more, so that an event on some thread is aware of some $\wevent$, only if there is a path on the execution graph involving exclusively $\porel$ and $\rfrel$ edges. 
%

As we remove edges from the paths corresponding to each memory model, we practically allow for read events to read from more write events on other threads. Thus the memory models are weakened. 
We refer to \cite{DBLP:journals/toplas/LahavB22} for a more analytical discussion on these models and example execution graphs. 
%
%\begin{figure}
%\scalebox{0.7}{
%\begin{subfigure}[b]{0.45\textwidth}
%%\scalebox{0.65}{
%    \begin{tikzpicture}          
%        \node (w0) at (0,4) {$\eventof\wtype{\theta_1}{x}{a_0}$};
%        \node (w1) at (0,2) {$\eventof\wtype{\theta_1}{x}{a_1}$};
%        \node (w2) at (0,0) {$\eventof\wtype{\theta_1}{y}{b_1}$};
%
%        \node (ry) at (4,2) {$\eventof\rtype{\theta_2}{y}{b_1}$};
%        \node (rx) at (4,0) {$\eventof\rtype{\theta_2}{x}{a_0}$};
%
%        \draw[-stealth, \pocolor] (w0) -- (w1) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, \pocolor] (w1) -- (w2) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, \pocolor] (ry) -- (rx) node[midway, fill=white] {$\porel$};
%        
%        \draw[-stealth, dashed] (w0) -- (rx) node[midway, fill=white] {$\rfrel$};
%        \draw[-stealth, dashed] (w2) -- (ry) node[midway, fill=white] {$\rfrel$};
%    \end{tikzpicture}
%%}
%\caption{An execution graph violating $\wrasem$}
%\label{fig:WRA_violation}
%\end{subfigure}
%\begin{subfigure}[b]{0.45\textwidth}
%%\scalebox{0.65}{
%    \begin{tikzpicture}
%        \node (w1) at (7,2) {$\eventof\wtype{\theta_1}{x}{a_1}$};
%        \node (r2) at (7,0) {$\eventof\rtype{\theta_1}{x}{a_2}$};
%        \node (w2) at (11,2) {$\eventof\wtype{\theta_2}{x}{a_2}$};
%        \node (r1) at (11,0) {$\eventof\rtype{\theta_2}{x}{a_1}$};
%
%        \draw[-stealth, \pocolor] (w1) -- (r2) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, \pocolor] (w2) -- (r1) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, dashed] (w1) -- (r1) node[near start, fill=white] {$\rfrel$};
%        \draw[-stealth, dashed] (w2) -- (r2) node[near start, fill=white] {$\rfrel$};
%        \draw[-stealth, dashed, \cocolor] (w1) to[bend left] node[midway, fill=white] {$\xcorel{x}$} (w2);
%        \draw[-stealth, dashed, \cocolor] (w2) to node[midway, fill=white] {$\xcorel{x}$} (w1);      
%    \end{tikzpicture}
%%}
%\caption{An execution graph violating $\rasem$}
%\label{fig:RA_violation}
%\end{subfigure}
%\begin{subfigure}[b]{0.45\textwidth}
%%\scalebox{0.65}{
%        \begin{tikzpicture}
%        \node (w1x) at (0,4) {$\eventof\wtype{\theta_1}{x}{a_1}$};
%        \node (w1y) at (0,2) {$\eventof\wtype{\theta_1}{y}{b_2}$};
%
%        \node (r1) at (0,0) {$\eventof\rtype{\theta_1}{y}{b_1}$};
%        
%        \node (w2y) at (4,4) {$\eventof\wtype{\theta_2}{y}{b_1}$};
%        \node (w2x) at (4,2) {$\eventof\wtype{\theta_2}{x}{a_2}$};
%        \node (r2) at (4,0) {$\eventof\rtype{\theta_2}{x}{a_1}$};
%
%        \draw[-stealth, \pocolor] (w1x) -- (w1y) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, \pocolor] (w1y) -- (r1) node[midway, fill=white] {$\porel$};
%        
%        \draw[-stealth, \pocolor] (w2y) -- (w2x) node[midway, fill=white] {$\porel$};
%        \draw[-stealth, \pocolor] (w2x) -- (r2) node[midway, fill=white] {$\porel$};
%        
%        \draw[-stealth, dashed] (w1x) -- (r2) node[near end, fill=white] {$\rfrel$};
%        \draw[-stealth, dashed] (w2y) -- (r1) node[near end, fill=white] {$\rfrel$};
%        
%        \draw[-stealth, dashed, \cocolor] (w1y) to node[near end, fill=white] {$\xcorel{y}$} (w2y);
%        \draw[-stealth, dashed, \cocolor] (w2x) to node[near end, fill=white] {$\xcorel{x}$} (w1x);
%        \end{tikzpicture}
%% }
%\caption{An execution graph violating $\srasem$}
%\label{fig:SRA_violation}
%\end{subfigure}
%}
%\caption{Some small execution graphs that provide characteristic litmus-test examples that separate our memory models. For each execution graph, the stated model is the \textit{stronger} violated one. }
%\label{fig:memory_model_examples}
%\end{figure}


\subsection{Consistency Models}
\label{sec:weak_memory_models}
\begin{definition}\label{def:egraph_satisfies_memory_model}
    Let $\egraph=\tuple{\events,\porel,\rfrel,\partcorel}$ be a (possibly partial) execution graph. 
    \begin{itemize}
        \item We write $\egraph\models\wrasem$ to denote that the relation $\mkrelof{\wtype}\cdot\hbrel\cdot\wevent\cdot\hbrel\cdot\invmkrelof\rfrel$ is acyclic.
        \item We write $\egraph\models\rasem$ to denote that the relation $\tclosureof{\mkrelof{\porel\cup\rfrel\cup\partcorel_{\xvar}}}$ is acyclic  for each variable $\xvar\in\varset$. 
        \item We write $\egraph\models\srasem$ to denote that the relation $\tclosureof{\mkrelof{\porel\cup\rfrel\cup\partcorel}}$ is acyclic. 
    \end{itemize}
\end{definition}
%rsp. $\srasem$, and $\wrasem$),  (rsp. the relation $\porel\cup\rfrel\cup\corel$ and the relation $(\porel\cup\rfrel)^+\cdot\wevent\cdot(\porel\cup\rfrel)^*\cdot\invmkrelof\rfrel$ is acyclic).
%
For a set  $\events$  of events, a program-order relation $\porel$ on $\events$, and a reads-from relation $\rfrel$ on $\events$, we write $\tuple{\events,\porel,\rfrel}\models\rasem$ if there is a total coherence-order relation $\corel$ on $\events$ such that $\tuple{\events,\porel,\rfrel,\corel}\models\rasem$ (rsp. $\srasem$, and $\wrasem$).
%
We write $\tuple{\events,\porel}\models\rasem$ if there is a reads-from relation $\rfrel$ and a coherence-order relation $\corel$ on $\events$ such that $\tuple{\events,\porel,\rfrel,\corel}\models\rasem$ (rsp. $\srasem$, and $\wrasem$).
%
\begin{definition}[Memory models over runs]
\label{def:run_satisfies_memory_model}
    For a run $\run$, we write $\run\models\rasem$ to denote that there exists a partial execution graph $\egraph_{\run}$, such that $  \tuple{\initconf,\egraph_{\emptyset}} \cmovesto{\run}  \tuple{\conf_1,\egraph_{\run}} $, and $\egraph_{\run} = \tuple{\events,\porel,\rfrel,\partcorel}$, and there exists a total coherence-order relation $\corel$, with $\partcorel \subseteq \corel$, such that $\egraph_t = \tuple{\events,\porel,\rfrel,\corel} \models \rasem$. 
%    $\egraph_{\run}\models\rasem$
 %       We define as $\porel,\rfrel,\partcorel$ of a run $\run$ to be the relations of $\egraph$ such that 
    (rsp. $\srasem$, and $\wrasem$). 
\end{definition}
\begin{definition}[Memory models over register machines]
\label{def:rmachine_satisfies_memory_model}
For a register machine $\rmachine$, we write $\rmachine\models\rasem$ if $\forall\run\in\runsetof\rmachine.\;\run\models\rasem$.      (rsp. $\srasem$, and $\wrasem$). 
%
\end{definition}
In other words, a register machine satisfies the $\rasem$-semantics if all its runs satisfy $\rasem$. 
Now that we have defined the memory models we will study we are ready to prove the following: 
%
\begin{lemma}\label{lem:partial_co_to_total_co}
    Assume a register machine $\rmachine$ and $\run \in\runsetof\rmachine$. Then, for  $  \tuple{\initconf,\egraph_{\emptyset}} \cmovesto{\run}  \tuple{\conf_1,\egraph_{\run}} $, with $\egraph_{\run} = \tuple{\events,\porel,\rfrel,\partcorel}$. 
    If $\egraph_{\run} \models \rasem$, then there exists total coherence order $\corel$, with $\partcorel \subseteq \corel$, such that $\egraph_t = \tuple{\events,\porel,\rfrel,\corel} \models \rasem$. (rsp. $\srasem$, and $\wrasem$). 
\end{lemma}
%
The above lemma guarantees that if for all runs $\run$ of a register machine $\rmachine$, $\egraph_{\run} \models \rasem$, then $\rmachine\models\rasem$ as well. 
We will only prove this in the case of $\rasem$, as a similar construction works for all the memory models in this paper. 
\begin{proof} 
    Assume a register machine $\rmachine$ and $\run \in\runsetof\rmachine$, and let $  \tuple{\initconf,\egraph_{\emptyset}} \cmovesto{\run}  \tuple{\conf_1,\egraph_{\run}} $, with $\egraph_{\run} = \tuple{\events,\porel,\rfrel,\partcorel}$ for some partial execution graph $\egraph_{\run}$. 
    Let $\wevent, \wevent'$ be two write events on the same variable $\xvar$, such that $(\wevent,\wevent'), (\wevent',\wevent) \not\in \partcorel_x$. 
    If either $(\wevent,\wevent')$, or $ (\wevent',\wevent) \in\mkrelof{\partcorel_{\xvar} \cup \porel\cup \rfrel}^+$, then we append the pair to $\partcorel$ edge that respects the direction of this path and we are done. 
    Otherwise, if $\wevent, \wevent'$ are incomparable w.r.t. $\mkrelof{\partcorel_{\xvar} \cup \porel\cup \rfrel}^+$ then we pick such events that are locally maximal for $\tclosureof{\mkrelof{\porel\cup\rfrel\cup\partcorel_{\xvar}}}$.
    %From the rules of \cref{fig:exec_graph_transitions}, this can only be the case if there is no read event $\revent$ in $\egraph_{\run}$, for which $\wevent \mkrelof\rfrel \revent$, and $\wevent' \mkrelof{\porel \cup \rfrel} \revent$ (or symmetrically). 
    In this case, it is safe to pick at random one of $(\wevent,\wevent'), (\wevent',\wevent)$ and add to $\partcorel_{\xvar}$ as no cycles will be introduced. 
    We continue the above process until we are left with a total $\corel$ for each variable $\xvar$, and we are done. 
    The construction for $\wrasem$ and $\srasem$ is identical, with the modification that we consider $\mkrelof{\cup \porel\cup \rfrel}^+$, and $\mkrelof{\partcorel\cup \porel\cup \rfrel}^+$ paths, respectively. 
\end{proof}
\subsection{Verification Problems}\label{prob:RA}
We write $\rmachine\xmodels\difftype\rasem$ if $\forall\run\in\diffrunsetof\rmachine.\;\run\models\rasem$. I.e., in the latter case,  we only consider the set of differentiated runs (rather the set of all runs). 
Note that for differentiated runs, the transition rules of  \cref{add:event:fig} become deterministic without the use of \cref{run:egraph:fig}. 
 
An instance of $\raconsprob$ consists of a register machine $\rmachine$, and the task is to decide whether $\rmachine\models\rasem$. 
Similarly,  an instance of $\sraconsprob$ consists of a register machine $\rmachine$, and the task is to decide whether $\rmachine\models\srasem$, and an instance of $\wraconsprob$ consists of a register machine $\rmachine$, and the task is to decide whether $\rmachine\models\wrasem$.
%
In $\radiffconsprob$, the task is to decide whether $\rmachine\xmodels\difftype\rasem$.

\begin{lemma}\label{lem:RA_to_diff_RA}
$\raconsprob$ is reducible to $\radiffconsprob$.
\end{lemma}

\begin{proof}
    We observe that the register machine model is inherently data independent ( \cite{DBLP:conf/popl/BouajjaniEGH17},\cite{POPL_Wolper86_data_independence}). 
    We argue that if a non-differentiated run exists that violates the $\rasem$, then so does a differentiated one.
    To demonstrate this, for any arbitrary $\rmachine$ and $\run \in\runsetof\rmachine$, with $  \tuple{\initconf,\egraph_{\emptyset}} \cmovesto{\run}  \tuple{\conf_1,\egraph_{\run}} $, we assume $\egraph_{\run} \not\models\rasem$. 
    Note that the transition $\cmovesto{\run}$ is non-deterministic. 
    We now create a new run $\run'$, by defining a meta-counter of steps taken in $\run$, and append that counter followed by a $\#$ to all values written in the memory. 
    The new run is now differentiated, which means that $\cmovesto{\run'}$ is deterministic, and the register machine $\rmachine$ must take identical transitions while processing it (since it is data independent). 
    Thus we would get that the resulting execution graph is identical to $\egraph_{\run}$, and thus also would be a violating one. 
    
    %f we assume there exists a run that violates any of our memory models, we can apply the same argument to transform it into a differentiated run. 
     In the converse direction, if a differentiated run violates a semantic model, the same run is a valid run of the register machine without the meta-variable modification. 
    Thus $\rmachine\models\rasem$ iff $\rmachine\xmodels\difftype\rasem$ (rsp. $\wrasem$ or $\srasem$), and we are done.  
\end{proof}

The above can be similarly extended for $\wraconsprob$ and $\sraconsprob$.

==> rmachines.tex <==
In this section, we will formally introduce the model of register machines and define its operational semantics.
%
%
We will use the following notation:
\begin{itemize}
    \item  Given a relation $\rel$, $\fundomof\rel$ denotes its domain; $\rclosureof\rel$. 
and $\tclosureof\rel$  denote its
reflexive and transitive closures; and $\invmkrelof\rel$
denotes its inverse. 
    \item Given a function $\fun$, we write
    $\updatefun\fun{\xvar}{\yvar}$, to denote a new function $\fun'$, where $\fun'(\xvar)=\yvar$, and $
    \fun'(\xvar')=\fun(\xvar')$, if $\xvar' \neq \xvar$.
    \item Given an expression $S$, we denote as 
$S(\sfrac{a}{b})$, the expression $S$, where all occurrences of $b$ have been replaced with $a$. Note that if $S$ had no occurrences of $b$ then $S(\sfrac{a}{b}) = S$.
    \item For a set $\mathcal{S}$ and an element $a$, we define $\mathcal{S}\oplus a$ to be a new set $\mathcal{S}'$ which is equal to $\mathcal{S}$ but also contains $a$. 
Note that $\mathcal{S}' = \mathcal{S}$ if $a \in \mathcal{S}$.
\end{itemize}

\subsection{Model}
\label{rmachines:mode:subsection}
Assume a set $\threadset$ of threads, a set $\varset$ of variables, and a set $\regset$ of registers.
%
We assume that the variables and the registers range over a (potentially infinite) set $\valset$ of data values with the particular value $\zero\in\valset$.
%
A {\it register machine} (or simply a {\it machine}) $\rmachine$ is a tuple $\rmachinetuple$ where $\stateset$ is the finite set of states, $\initstate\in\stateset$ is the initial state, and $\transitionset$ is the finite set of transitions.
%
A transition is a triple of the form $\tuple{\mystate,\op,\pqstate}$ where $\mystate,\pqstate\in\stateset$ are states, and $\op$ is an operation.
%
The operation $\op$ can be in one of the following three forms:
\begin{itemize}
\item
$\wopof\thread\xvar\areg$ receives the value of the variable $\xvar$ from $\thread$ and writes (stores) the value in register $\areg$.
%
The environment selects the written value (the program running on $\rmachine$).
%
\item
$\ropof\thread\xvar\areg$ reads of value of the variable $\xvar$ from the register $\areg$ and delivers the stored value to $\thread$.
\item
$\areg\assigned\areg'$ copies the value stored in the register $\areg'$ to the register $\areg$.
\end{itemize}

For any register machine, it is clear we can pre-process it to omit any unreachable states. We state and prove all remaining algorithms after this pre-processing has taken place, and thus with all remaining register machine states being reachable. 

% we will assume that all states in a register machine are reachable. This can be easily verified for any register machine, and if there are unreachable states, we can remove them. 

\subsection{Operational Semantics}
\label{op:sem:subsection}
%
We define the operational semantics of a register machine by defining the transition system it induces, i.e., by defining the set of configurations of the machine together with a transition relation on them.\footnote{We use the term {\it transition} to refer both to the set of transitions in the syntax of the machine (\cref{rmachines:mode:subsection}) and to the transition relation on configurations (here in \cref{op:sem:subsection}). The meaning will always be clear from the context.}
A {\it configuration} $\conf$ is of the form $\tuple{\mystate,\regvalmapping}$ where $\mystate\in\stateset$ defines the state of the machine, and $\funtype\regvalmapping\regset\valset$ defines the value $\regvalmappingof\areg$ of each register $\areg\in\regset$.
%
The \textit{initial configuration} $\initconf$ is the pair $\tuple{\initstate,\lambda\,\regset.\,\zero}$, i.e., the machine $\rmachine$ starts running from a configuration where it is in its initial state and all its registers contain the value $\zero$.
%
We use $\confset$ to denote the set of configurations.

%

\begin{figure}
\centering
\begin{gather*}
\scalebox{0.75}{
\threeinfer
    { \text{Write}}{
      \tuple{\mystate,\wopof\thread\xvar\areg,\pstate}
      \in\transitionset
      }
    {
      \val\in\valset\;\;\;\pregvalmapping=\updatefun\regvalmapping\avar\val
    }
    {
      \tuple{\mystate,\regvalmapping}
      \rmovesto\rmachine{\weventof\thread\xvar\areg\textcolor{red}{\sslash\val}}{}
      \tuple{\pstate,\pregvalmapping}
    }
}
\irspace
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\scalebox{0.75}{\threeinfer{\text{Read}}
    {
      \tuple{\mystate,\outopof\thread\xvar\areg,\pstate}
      \in\transitionset
      }
    {
      \regvalmappingof\avar=\val
    }
    {
      \tuple{\mystate,\regvalmapping}
      \rmovesto\rmachine{\reventof\thread\xvar\areg\textcolor{red}{\sslash\val}}{}
      \tuple{\pstate,\regvalmapping}
    }
}\irspace
\scalebox{0.75}{\threeinfer{\text{Copy}}
    {
      \tuple{\mystate,\areg\assigned\areg',\pstate}
      \in\transitionset
      }
    {
      \pregvalmapping=
      \updatefun\regvalmapping
          {\areg}{\regvalmappingof{\areg'}}
    }
    {
      \tuple{\mystate,\regvalmapping}
      \rmovesto\rmachine{\silentevent}{}
      \tuple{\pstate,\pregvalmapping}
    }
}
\end{gather*}
  \caption{The semantics of a register machine's three operations. Write and copy operations update the state of the memory $\regvalmapping$, while read operations only update the state of the register machine. }
  \label{fig:semantics_exec_graphs}
\end{figure}
%
A transition is of the form $\iconf1\movesto\action\iconf2$ where $\iconf1,\iconf2\in\confset$ are configurations, and $\action$ is an operation, potentially augmented with a concrete value to be read or written.
%
We define the transition relation according to Figure \ref{fig:semantics_exec_graphs} inference rules.
%
In the write rule, the machine executes a transition from $\mystate$ to $\pstate$ while processing a write operation.
%
The configuration changes state accordingly and updates the value of the relevant register as implied by the operation.
%
In the read rule, the machine processes a read operation that returns the relevant register's value.
%
%The transition is labeled by a real event whose parameters are decided by the output operation. 
%
The machine performs a register assignment operation in the copy rule.
%
The operation is not visible to the external threads; hence, it is labeled by the silent event $\silentevent$. 
%
As we shall see later, the actual value $\val$ that $\thread$ writes/reads  to/from $\xvar$ is not relevant for our analysis; nevertheless, we include it in the transition label for clarity.

A run $\run$ of the program is a sequence $\iconf0\movesto{\iop1\sslash\ival1}\iconf1\movesto{\iop2\sslash\ival2}\cdots\movesto{\iop\nn\sslash\ival\nn}\iconf\nn$ of transitions.
%
Sometimes, when the states and the values are not relevant in the context, we simply represent $\run$ as the sequence of operations $\iop1\iop2\cdots\iop\nn$.
%
We say that $\run$ is initialized if $\iconf0=\initconf$, i.e., the run starts from the initial configuration.
%
We use $\runsetof\rmachine$ to denote the set of all initialized runs of $\rmachine$.
%





